Learning Rich Representation of Keyphrases from Text

In this work, we explore how to train task-specific language models aimed towards learning rich representation of keyphrases from text documents. We experiment with different masking strategies for pre-training transformer language models (LMs) in discriminative as well as generative settings. In the discriminative setting, we introduce a new pre-training objective - Keyphrase Boundary Infilling with Replacement (KBIR), showing large gains in performance (upto 8.16 points in F1) over SOTA, when the LM pre-trained using KBIR is fine-tuned for the task of keyphrase extraction. In the generative setting, we introduce a new pre-training setup for BART - KeyBART, that reproduces the keyphrases related to the input text in the CatSeq format, instead of the denoised original input. This also led to gains in performance (upto 4.33 points in F1@M) over SOTA for keyphrase generation. Additionally, we also fine-tune the pre-trained language models on named entity recognition (NER), question answering (QA), relation extraction (RE), abstractive summarization and achieve comparable performance with that of the SOTA, showing that learning rich representation of keyphrases is indeed beneficial for many other fundamental NLP tasks.

==> methodology.tex <==
\section{Keyphrase Language Modeling}
% \label{sec:method}

% We train transformer based language models with various settings to learn good representations of keyphrases. Our model architectures follow RoBERTa and BART for extractive and generative approaches respectively. We change their pre-training objectives by introducing different masking strategies. In this effort we introduce 
% The language model objective as introduced in BERT \cite{devlin2018bert} perform pre-training by maximizing the log-likelihood:

% \begin{equation}
% \label{eq:mlm}
% \mathcal{L}_{\mathrm{MLM}}(\boldsymbol{\theta})=\sum_{i=1}^{n} m_{i} \log p\left(x_{i} \mid \boldsymbol{x} \circ \boldsymbol{m} ; \boldsymbol{\theta}\right)
% \end{equation}

% where, $x = [x_{1}, ... ,x_{n}]$ is the original sequence of tokens, $\circ$ denotes the element-wise product, and $m = [m_{1}, ... ,m_{n}]$ is the binary vector where $m_{i} = 1$ indicates replacing $x_{i}$ with $[$MASK$]$ or otherwise unchanged. $\theta$ represent the model parameters. The MLM method learns rich contextual representation of tokens. 

% In order to learn better contextual representation of keyphrases, we introduce the Keyphrase Language Modeling (KLM) objective, in which we not only mask tokens as in MLM, but also mask keyphrases in a given context. $m$ is replaced by $m^{'} = [m^{'}_{1}, ... ,m^{'}_{n}]$, which is a binary vector having a contiguous sequence of $[$MASK$]$ representing masking of keyphrases along with random masking of a non-keyphrase tokens, as shown in Fig \ref{fig:masking-strategies}.

% The keyphrases are identified using an unsupervised keyphrase extraction algorithm.  


% We explore extending work in \cite{ye2018semi} by leveraging unsupervised keyphrase extraction techniques in pre-training language models. We run TextRank (Mihalcea et al., 2004) <Add citation> on the Wikipedia <Add Citation> and S2ORC <Add Citation> corpus to tag keyphrases at a large scale and this tagged corpus serves as our base dataset. 

% \subsection{Masking Strategies}

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/Setups.PNG}
%     \caption{Masking Strategies, the keyphrase present in the text are highlighted in Purple and every perturbation in the form of a random MASK is represented in Red, keyphrase MASK is represented in Blue and Keyphrase Replacement is represented in Gold.}
%     \label{fig:masking-strategies}
% \end{figure*}

\subsection{Token Masking}
The language model objective as introduced in BERT \cite{devlin2018bert} perform pre-training by maximizing the log-likelihood:

\begin{equation}
\label{eq:mlm}
\mathcal{L}_{\mathrm{MLM}}(\boldsymbol{\theta})=\sum_{i=1}^{n} m_{i} \log p\left(x_{i} \mid \boldsymbol{x} \circ \boldsymbol{m} ; \boldsymbol{\theta}\right)
\end{equation}

where, $x = [x_{1}, ... ,x_{n}]$ is the original sequence of tokens, $\circ$ denotes the element-wise product, and $m = [m_{1}, ... ,m_{n}]$ is the binary vector where $m_{i} = 1$ indicates replacing $x_{i}$ with $[$MASK$]$ or otherwise unchanged. $\theta$ represent the model parameters. The MLM method learns rich contextual representation of tokens. We associate $\alpha$ as a loss weighting coefficient for the token masking objective.

% \subsubsection{Keyphrase Masking}
% While \cite{joshi2020spanbert} explores masking entities, random spans and noun-phrases they do not explore masking keyphrases. Further the success of entity masking and prediction demonstrated in by \cite{yamada2020luke} serves as motivation to further extending token masking strategies. Different from these previous approaches rather than masking individual tokens in a span we replace the entire keyphrase span with a single [MASK] token.

\subsection{Keyphrase Boundary Infilling} 
\label{subsec:kbi}
In order to effectively learn richer representations of keyphrases we propose a new pre-training objective that is inspired by the Span Boundary Objective from \cite{joshi2020spanbert} and the text infilling setup from \cite{lewis2019-bart}. Instead of replacing each of the individual tokens of the span with a [MASK] token, similar to \cite{lewis2019-bart} we replace the entire span, in this case a keyphrase, with a [MASK] token. Text infilling to the best of our knowledge has not been explored in a discriminative setup and we propose to predict the original tokens by using positional embeddings in the text in conjunction with the boundary tokens. However, we limit the maximum number of tokens that can be produced since unlike the Span Boundary Objective we do not know the actual number of tokens.

Similar to the Span Boundary Objective, we denote the output of the transformer encoder for each token in the sequence by $x_{1}, . . . , x_{n}$. However since the entire span of tokens $(x_{s}, . . . , x_{e}) \in Y$ is masked it is represented with a single $x_{m}$, where $(s, e)$ indicates its start and end positions and $m$ represents the index of the masked spans. We set a  maximum possible number of tokens corresponding to a span, $MT$ such that $i \in (1, MT)$. We then expand potential tokens present in $x_{m}$ using the output encodings of the external boundary tokens $x_{s-1}$ and $x_{e+1}$, as well as the position embedding of the target token $p_{i-s+1}$:

\begin{equation}
\label{eq:infill-y}
y_{i} = f(x_{s-1}, x_{e+1}, p_{i-s+1})
\end{equation}

where position embeddings $p_{1}, p_{2}, . . .$ mark relative positions of the masked tokens with respect to the left boundary token $x_{s-1}$. We use the Layer Normalization \cite{ba2016-layer-norm} and GeLU \cite{gelu-hendrycks2016} activation functions similar to the Span Boundary Objective to represent $f(\Delta)$.

We then use the vector representation $y_{i}$ to predict the potential token $x_{i}$ from the unmasked $x_{m}$ and compute the cumulative cross-entropy loss for each $i$ present within the unmasked $x_{m}$.
\begin{equation}
\label{eq:infill}
\mathcal{L}_{\mathrm{Infill}}(\boldsymbol{\theta})=\sum_{i=1}^{MT} \log p\left(x_{i} \mid\boldsymbol{y_{i}}\right)
\end{equation}

Further we set this up as a multi-task learning setup where in addition to predicting the actual tokens, a classification head must predict the expected number of tokens corresponding to this [MASK] in the anticipation of providing a stronger learning signal. Each possible length of the [MASK] is represented as a class up to the maximum number of tokens possible. This architecture used is a single linear layer which is trained with cross-entropy loss $\mathcal{L}_{\mathrm{LP}}(x_{m}, z_{m})$ with the infilled masked token $x_{m}$ and the corresponding actual length of the span class $z_{m}$. 

The Keyphrase Boundary Infilling (KBI) pre-training objective objective is formally represented as: 
\begin{equation}
\label{eq:sbi}
\mathcal{L}_{\mathrm{KBI}}(\boldsymbol{\theta})= \gamma \mathcal{L}_{\mathrm{Infill}}(\boldsymbol{\theta}) + \sigma\mathcal{L}_{\mathrm{LP}}(\boldsymbol{\theta})  
\end{equation}

where the $\gamma$ and $\sigma$ are hyperparameters for co-efficients applied to each loss.

\subsection{Keyphrase Replacement}
\label{subsec:keyphrase_replacement}
WKLM \cite{xiongetal2019-wklm} also explores pretraining a language model through weak supervision by replacing entities with random entities of the same type that were a part of the knowledge base. We adapt this to replace keyphrases by randomly choosing another keyphrase of variable length from the universe of keyphrases identified in the tagged corpus. The replacement classification task is modeled as a binary classification task to determine if a keyphrase is replaced or the original, by concatenating the keyphrase boundary tokens representation as inputs to learn a linear classifier. We associate $\delta$ as a loss weighting coefficient for the keyphrase replacement objective.
%Representing spans via their boundary tokens has been explored in SpanBERT \cite{joshi2020spanbert}, WKLM \cite{xiongetal2019-wklm} and \cite{yu2020-ner-dependency-parse}.

% Once again, consider the output of the transformer encoder for each token in the sequence by $x_{1}, . . . , x_{n}$. We identify tokens $x_{sk}, ..., x_{ek}$ to represent a keyphrase where $(sk, ek)$ represent the start index and end index for the keyphrase. We use the concatenated representation of boundary tokens of $x_{sk-1}$ and $x_{ek+1}$ as input to the linear layer. Given the label $y_{k}$ representing whether a keyphrase was replaced or not the training loss here is simply represented as a binary cross-entropy loss $\mathcal{L}_{\mathrm{REP}}((x_{sk-1} + x_{ek+1}) , y_{k})$.

\subsection{KeyBART}
\label{subsec:keybart}
Inspired by BART \cite{lewis2019-bart}, where they explore generating sequences of different lengths from the input perturbed with [MASK] tokens along with token addition and deletion. We differently explore generating rich keyphrase representations by attempting to generate the original keyphrases in the Catseq format as proposed in \cite{meng-etal-2017-deep} from an input perturbed with Token Masking, Keyphrase Masking and Keyphrase Replacement. We maintain the order of occurrence of the keyphrases in the original document and we also remove duplicate occurrences of keyphrases. Similar to BART we use a reconstruction loss objective during training which is a cross-entropy loss between the output and set of expected keyphrases.

% \textbf{We tweak the strategy as implemented in \cite{he2020kgplm}, by replacing the knowledge sensitive spans with keyphrases in our case. Please note that this section has to be re-written.}


% we use a combined generative and discriminative approach as introduced in ELECTRA \cite{clark2020electra}. The generative approach makes the model predict the masked tokens that are part of a keyphrase as shown in Figure \ref{}. Formally, with the masking scheme $m^{K}$ induced by the keyphrases, the masked sequence now becomes $\overline{x} = KLM-MASK(x) = x \circ m^{K}$. The generative loss as given by equation \ref{eq:2} is then defined as the negative log-likelihood of predicting the masked tokens:

% \begin{equation}
% \label{eq:2}
%     \mathcal{L}_{\mathrm{Gen}}\left(\boldsymbol{\theta}_{g}\right)=-\sum_{i=1}^{n} m_{i}^{\mathcal{K}} \log p\left(x_{i} \mid \overline{\boldsymbol{x}} ; \boldsymbol{\theta}_{g}\right)
% \end{equation}

% In the discriminative approach the original sequence is converted to $\hat{x} = KLM-Replace(x)$ by replacing the tokens of a keyphrase with another semantically unrelated keyphrase. Discriminative loss could be defined at sequence-level, span-level, or token-level \todo{we need to talk a little about our experience of training at span-level}. In this paper, we use the fine-grained token-level loss, which is the cross-entropy loss of classifying whether the token is replaced or not as shown in equation \ref{eq:3}:

% \begin{equation*}
% \label{eq:3}
%     \begin{aligned*}
%     \mathcal{L}_{\mathrm{Disc}}\left(\boldsymbol{\theta}_{d}\right)=- \sum_{i=1}^{n} \mathbb{1}\left(\hat{x}_{i}=x_{i}\right) \log p\left(r_{i}=0 \mid \hat{\boldsymbol{x}} ; \boldsymbol{\theta}_{d}\right) \\
%     &+\mathbb{1}\left(\hat{x}_{i} \neq x_{i}\right) \log p\left(r_{i}=1 \mid \hat{\boldsymbol{x}} ; \boldsymbol{\theta}_{d}\right)
%     \end{aligned*}
% \end{equation*}

% Here each $r_{i}$ is binary variable indicating whether $\hat{x_{i}}$ is different from $x_{i}$. Figure \ref{} illustrates our framework. The proposed keyphrase guided pre-training, could then be defined as the following optimization problem:

% \begin{equation}
%     \min _{\boldsymbol{\theta}_{g}, \boldsymbol{\theta}_{\boldsymbol{d}}} \mathcal{L}_{\mathrm{Gen}}\left(\boldsymbol{\theta}_{g}\right)+\lambda \mathcal{L}_{\mathrm{Disc}}\left(\boldsymbol{\theta}_{d}\right)
% \end{equation}

% \subsection{Generative Pre-training}
% Given the input sequence $x_{i}$, unlike the conventional random masking, we particularly extract the spans of text that are assigned as keyphrases. In this work, we used three large datasets - OAGKX, KP20K and KPTimes (see Section \ref{sec:data}) annotated with keyphrases. All the datasets were combined in order to get a large corpus with annotated keyphrases across a diverse set of topics spanning across the different domains of scientific research and news articles \todo{Need to give a detailed account of the dataset along with some useful stats}. However, the datasets consists of both abstractive (not part of the document) as well as extractive keyphrases (part  of the document). During masking we only consider extractive keyphrases. 

% Give an example and explain it. Also mention that instead of considering a short sequence equivalent to avg. length of sentences we consider a sequence of $x$ tokens. The number x needs to come from the max length of tokens that

% In practice, since the coverage of keyphrases can vary in different input sequences, we use a mixture of keyphrase masking and subword masking., while still keeping the total mask ratio of 15\%. Specifically, a probabilistic masking strategy is designed to choose whether to mask a keyphrase span or a subword \todo{are we going to use subword or a subsequence of tokens?} every time. For each input text sequence, keyphrase spans (if available) or subwords are masked iteratively by following the strategy until reaching the masking ratio of 15\%.

% \subsection{Discriminative Pre-training}

% In the discriminative pre-training part we randomly replace a keyphrase from an input sequence by another keyphrase of the same length. In this process we use two different strategies - a. replacement keyphrase is semantically similar, b. replacement keyphrase is semantically dissimilar. This is achieved by randomly selecting a same-length entry from the keyphrase vocabulary and then getting its vector representation using a Word2Vec model \todo{we will have to add details of the Word2Vec model} trained on our corpus. Half of the time we select a keyphrase for replacement that is semantically dissimilar from the candidate by setting a threshold of 0.1 for the cosine similarity score, and for the other half of the time we choose a replacement keyphrase that has more than 0.9 cosine similarity with the candidate. The discrimnator's task is to distinguish which tokens or a sequence of tokens are replaced $(r_{i} = 1)$, and which are not $(r_{i} = 0)$.

% We give an example.


% For each token the probability of being replaced is computed as:

% \begin{equation}
%     p\left(r_{i} \mid \hat{\boldsymbol{x}} ; \boldsymbol{\theta}_{d}\right)=\operatorname{sigmoid}\left(w^{T} \operatorname{GeLU}\left(\boldsymbol{W} \boldsymbol{h}\left(\hat{x}_{i}\right)\right)\right.
% \end{equation}

% where $h(\hat{x_{i}})$ is the contextualized representation of $\hat{x_{i}}$, by the discriminator, which is a 12-layer Transformer encoder.

% In addition to keyphrase substitution, we also randomly replace some of the subwords with random tokens. The total replacement ratio of a sentence is kept at 15\%.


==> qualitative_analysis_table.tex <==
\begin{table*}[htbp]
\small
\centering
    \begin{tabular}{p{0.95\linewidth}}
    \hline
    \textbf{Input Text}: On The Complexity of Combinatorial Auctions : Structured Item Graphs and Hypertree Decompositions. The winner determination problem in combinatorial auctions is the problem of determining the allocation of the items among the bidders that maximizes the sum of the accepted bid prices. While this problem is in general NPhard, it is known to be feasible in polynomial time on those instances whose associated item graphs have bounded treewidth called structured item graphs. Formally, an item graph is a graph whose nodes are in one-to-one correspondence with items, and edges are such that for any bid, the items occurring in it induce a connected subgraph. Note that many item graphs might be associated with a given combinatorial auction, depending on the edges selected for guaranteeing the connectedness. In fact, the tractability of determining whether a structured item graph of a fixed treewidth exists and if so, computing one was left as a crucial open problem. In this paper, we solve this problem by proving that the existence of a structured item graph is computationally intractable, even for treewidth 3. Motivated by this bad news, we investigate different kinds of structural requirements that can be used to isolate tractable classes of combinatorial auctions. We show that the notion of hypertree decomposition, a recently introduced measure of hypergraph cyclicity, turns out to be most useful here. Indeed, we show that the winner determination problem is solvable in polynomial time on instances whose bidder interactions can be represented with dual hypergraphs having bounded hypertree width. Even more surprisingly, we show that the class of tractable instances identified by means of our approach properly contains the class of instances having a structured item graph. \\
    \hline
    \textbf{Extracted Keyphrases}: [combinatorial auctions]; [structured item graphs]; [hypertree decompositions]; [item graphs]; [treewidth]; [bidders]; [hose nodes]; [hypertree cyclicity]; [polynomial time] \\
    \textbf{Generated Keyphrases}: [combinatorial auctions]; [structured item graphs]; [treewidth]; [hypergraphs]; [hypertree decompositions] \\
    \textbf{Ground Truth}: [hypergraph]; [structured item graph]; [polynomial time]; [combinatorial auction]; [fixed treewidth]; [accepted bid price]; [hypertree decomposition]; structured item graph complexity; simplification of the primal graph; hypertree based decomposition method; hypergraph hg; the primal graph simplification; well known mechanism for resource and task allocation; complexity of structured item graph;  \\
    \hline
    \hline
    \textbf{Input Text}: Interesting Nuggets and Their Impact on Definitional Question Answering. Current approaches to identifying definitional sentences in the context of Question Answering mainly involve the use of linguistic or syntactic patterns to identify informative nuggets. This is insufficient as they do not address the novelty factor that a definitional nugget must also possess. This paper proposes to address the deficiency by building a Human Interest Model from external knowledge. It is hoped that such a model will allow the computation of human interest in the sentence with respect to the topic. We compare and contrast our model with current definitional question answering models to show that interestingness plays an important factor in definitional question answering. \\
    \hline
    \textbf{Extracted Keyphrases}: [interesting nuggets]; [definitional sentences]; [question answering]; [nuggets]; [novelty]; [definitional nuggets]; [human interest model]; [human interest] \\
    \textbf{Generated Keyphrases}: [definitional question answering]; natural language processing \\
    \textbf{Ground Truth}: [human interest]; [use of linguistic]; [interesting nugget]; [definitional question answer]; [informative nugget]; [interest]; [computation of human interest]; sentence fragment; unique quality; manual labor; news corpus; baseline system; human interest computation; human reader; linguistic use; question topic; external knowledge; surprise factor; lexical pattern \\
    \hline
    \hline
    \textbf{Input Text}: The Influence of Caption Features on Clickthrough Patterns in Web Search. Web search engines present lists of captions, comprising title, snippet, and URL, to help users decide which search results to visit. Understanding the influence of features of these captions on Web search behavior may help validate algorithms and guidelines for their improved generation. In this paper we develop a methodology to use clickthrough logs from a commercial search engine to study user behavior when interacting with search result captions. The findings of our study suggest that relatively simple caption features such as the presence of all terms query terms, the readability of the snippet, and the length of the URL shown in the caption, can significantly influence users ' Web search behavior. \\
    \hline
    \textbf{Extracted Keyphrases}: [influence]; [caption features]; [clickthrough patterns]; [web search]; [snippet]; [methodology]; [clickthrough logs] \\
    \textbf{Generated Keyphrases}: [web search]; [clickthrough]; [captions]; user study \\
    \textbf{Ground Truth}: [clickthrough pattern]; [snippet]; [web search behavior]; [web search]; [caption feature]; summarization; extractive summarization; significant word; query log; human factor; clickthrough inversion; query term match; query re formulation \\
    \hline
    \hline
    \end{tabular}
\caption{Sample keyphrases extracted by KBI-REP-CRF and generated by KeyBART on the SemEval-2010 dataset. Present keyphrases are marked with square brackets.}
\label{tab:qualitative_results}
\end{table*}


==> relatedwork.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Pre-training Objectives in Language Modeling}
% In the domain of natural language processing, pre-training and fine-tuning has become the new norm. Regardless of the target application (sentiment analysis, question answering, or machine translation), language models are first pre-trained on huge volumes of free-form text. The intention is to initialize models with general linguistic knowledge such as syntactic structures, lexical meaning, linguistic rules, semantics roles, etc that can be later leveraged for a variety of downstream tasks. Initially pretraining was used for learning word embeddings only, but due to its shallowness and inability to learn Contextual representation later most of the part of the model are pretrained and only few of the layer are fintuned on downstream tasks.

% Give an overview of different pre-training objectives and strategies. Masked Language Modeling, Next sentence prediction, Replace token detection (ELectra), paraphrasing, REALM,


\subsection{Keyphrase Identification}
% Keyphrases could either be \textit{extractive} (part of the document) or \textit{abstractive} (not part of the document). Some prior works have referred to them as present and absent keyphrases, respectively. Keyphrase generation is the process of predicting both extractive and abstractive keyphrases from a given document. Most of the previous works in keyphrase domain, including both supervised and unsupervised techniques, primarily focus on extractive keyphrases \cite{hasan2014automatic, mahata2018key2vec,sahrawat2020keyphrase}. Recent studies \citet{meng2017deep,ye2018semi,Chan2019NeuralKG} have started to develop generative approaches that produce both abstractive and extractive keyphrases from documents. Though these studies have shown some promise, the results suggest that there is great room for improvement.

% Give a brief overview of extractive keyphrases

% Give a brief overview of generative keyphrases

% Talk about some of the most recent works especially using Transformers like - TNT-KID, rui meng unsupervised generation work, etc. Recent work in COLING using Game Theoretical approach.

==> results.tex <==
\section{Results}
In this section we take a look at the impact of the various pre-training regimes on span-based downstream tasks, both classification and generation, that we hypothesis could benefit from richer keyphrase embeddings. We evaluate on tasks directly related to keyphrase such as Keyphrase Extraction and Keyphrase Generation. We also evaluate on Named Entity Recognition, Question Answering, Relation Extraction and Summarization.

 It is important to note that during inference our setups \textbf{do not use any additional parameters compared to RoBERTa for the Classification tasks or BART for the Generation tasks and just rely on richer token embeddings}.

\begin{table}[]
\scalebox{1.0} {
\begin{tabular}{lc}
\hline
\textbf{Model} & \textbf{F1}\\ \hline
LSTM-CRF (Lample et al., 2016) &  91.0 \\ 
ELMo (Peters et al., 2018)  & 92.2 \\ 
BERT (Devlin et al., 2019)  & 92.8 \\ 
Akbik et al. (2018) &  93.1 \\ 
Baevski et al. (2019) &  93.5 \\ 
LUKE (Yamada et al., 2020) &  \textbf{94.3} \\ 
LUKE w/o entity attention &  94.1 \\ \hline
RoBERTa            & 92.4  \\ 
RoBERTa-extended*   & 92.54   \\ 
RoBERTa-KLM*       & 92.73   \\ 
RoBERTa-KLM-REP*    & \textbf{\textit{92.97}}  \\ \hline
\end{tabular}
}
\caption{Named Entity Recognition results on  CONLL-2003. State-of-the-art is marked in \textbf{Bold} and our best performing models as \textbf{\textit{Bold-Italicized}}}
\label{tab:ner_results}
\end{table}

\subsection{Named Entity Recognition}
We study the performance of different models for the task of NER by conducting experiments on CoNLL-2003 dataset \cite{sang2003introduction}. We have used the sequence tagging Token Classification architecture implemented by \cite{wolf2020transformers} in order to fine-train different pre-trained models for the NER task. The architecture predicts token class types based on the output features generated by the model. For fine-tuning, we have used a learning rate of 1e-5 and the model is trained for 5 epochs on 1 GPU with a batch size of 8. Table \ref{tab:ner_results} reports F1 scores on the test set. Results demonstrate that the proposed models result in performance gains over RoBERTa on CoNLL-2003. With RoBERTa-extended, we see that only continued pre-training with the MLM objective results in minor gains. However, when we inspect the results for RoBERTa-KLM and RoBERTa-KLM-REP, we see consistent jumps in performance showing how both these architectures also contribute richer representations that directly impact NER performance. We hypothesize that RoBERTa-KLM-REP is more effective at NER than RoBERTa-KLM because the additional replacement classification task builds richer boundary token representations making entity identification potentially easier. The results are also fairly competitive with state-of-the-art NER literature despite this work not trying to model entities explicitly like the other work.

\begin{table}[]
\scalebox{1.0} {
\begin{tabular}{lcc}
\hline
Model & EM & F1 \\ \hline
BERT (Devlin et al., 2019) &  84.2 &  91.1 \\ 
XLNet (Yang et al., 2019) &  89.0 &  94.5 \\ 
ALBERT (Lan et al., 2020) &  89.3 &  94.8 \\ 
LUKE (Yamada et al, 2020) &  \textbf{89.8} &  \textbf{95.0} \\ 
LUKE w/o entity attention &  89.2 & 94.7 \\ \hline
RoBERTa             & 88.9 & 94.6 \\ 
RoBERTa-extended*   & 88.88 & 94.55    \\ 
RoBERTa-KLM*       & 88.97 & 94.7 \\ 
RoBERTa-KLM-REP*    & \textbf{\textit{89.04}} & \textbf{\textit{94.75}}  \\ \hline
\end{tabular}
}
\caption{Question Answering results on SQuAD v1.0 on the DEV set. State-of-the-art is marked in \textbf{Bold} and our best performing models as \textbf{\textit{Bold-Italicized}}}
\label{tab:qa_results}
\end{table}

\subsection{Question Answering}
The relation between Question Answering and Keyphrases has been explored in some capacity in \cite{subramanian-etal-2018-neural}, which leverages a keyphrase extractor to use for question generation. Motivated by this we evaluate our models on SQuAD v1.0 \cite{rajpurkar2016squad} dataset for the extractive question answering task. For all the models, we use a maximum sequence of length of 512 with a sliding window of size 128. In addition, model is fine-tuned with a learning rate of 3e-5 and batch size of 48 for 2 epochs. In order to achieve better reproducibility of results, we have used implementation by \cite{wolf2020transformers} for fine-tuning the models. Table \ref{tab:ner_results} reports the F1 and Exact Match (EM) scores achieved by different model architectures on the DEV set. We once again see improved performance with the proposed architecures of RoBERTa-KLM and RoBERTa-KLM-REP as compared to RoBERTa. We have a curious finding where RoBERTa-extended actually performs worse than RoBERTa and we think this is because of the domain shift in the pre-training data being focused on scientific articles. On the other hand, the models trained with keyphrase pre-training objectives are fairly competitive with the state-of-the-art Question Answering models. We explicitly include LUKE w/o entity attention since that removes the entity-aware attention module, making it slightly more comparable to our results. We see that RoBERTa-KLM-REP outperforms it by a slim margin on F1 however is slightly lower on the EM scores. We also highlight that our model's performance doesn't scale the same for EM as it does for F1 when compared to state-of-the-art, potentially explained by the model being more likely to identify keyphrases as answers. 

\begin{table}[]
\scalebox{1.0} {
\begin{tabular}{lc}
\hline
Model & F1\\ \hline
BERT (Zhang et al., 2019) & 66.0 \\
C-GCN (Zhang et al., 2018b) & 66.4 \\ 
ERNIE (Zhang et al., 2019) & 68.0 \\ 
SpanBERT (Joshi et al., 2020) & 70.8 \\ 
MTB (Baldini Soares et al., 2019) & 71.5 \\ 
KnowBERT (Peters et al., 2019) &  71.5 \\ 
KEPLER (Wang et al., 2019b) & 71.7 \\ 
K-Adapter (Wang et al., 2020)  & 72.0 \\ 
LUKE (Yamada et al., 2020) & \textbf{72.7} \\ 
LUKE w/o entity attention & 72.2 \\ \hline
RoBERTa            & 71.3  \\ 
RoBERTa-extended*  & 70.94   \\ 
RoBERTa-KLM*        & 70.71   \\ 
RoBERTa-KLM-REP*    & \textbf{\textit{71.0}}  \\ \hline
\end{tabular}
}
\caption{Relation Extraction results on TACRED. State-of-the-art is marked in \textbf{Bold} and our best performing models as \textbf{\textit{Bold-Italicized}}}
\label{tab:re_results}
\end{table}

\subsection{Relation Extraction}
The relation extraction task predicts relations among pairs of entity mentions in a text. 
We fine-tuned our models for the sentence-level relation extraction task using the popular TACRED benchmark dataset \cite{zhang-etal-2017-position}. TACRED contains more than 100,000 sentences with entities that belong to 23 different fine-grained semantic types and with 42 different relations among entities. To fine-tune our models, we modified the input sequences to mark the start and end of the subject entity with @ and the object entity with \#. We use the final layer representation of the [CLS] token as the input to a multi-class classifier. Similar to \cite{zhou2021improved}, we also observe that a model's performance depends heavily on the formatting of the input sequence. The results in the top half of Table~\ref{tab:re_results} are reported from the respective papers that use various different input formatting strategy. All models in the bottom half of the table are trained with the same input format mentioned above. We found a batch size of 32 and a learning rate between 2e-5 and 4e-5 to be optimal. We observe that our RoBERTa-KLM-REP model performs slightly worse than the original RoBERTa model. We also observe similar trends for RoBERTa-KLM and RoBERTa-extended models. We conjecture that the domain shift of the pretraining corpus is responsible for the slight performance degradation.

\begin{table}[]
\scalebox{0.85} {
\begin{tabular}{lcccc}
\hline
Model & Inspec & SE10 & SE17 \\ \hline
RoBERTa+BiLSTM-CRF         & 59.5 & 27.8 & 50.8  \\ 
RoBERTa+TG-CRF             & 60.4 & 29.7 & 52.1 \\ 
RoBERTa+Hypernet-CRF       & 62.3 & 34.8 & 53.3 \\ \hline
RoBERTa-extended-CRF*           & 62.09 & 40.61 & 52.32  \\ 
RoBERTa-KLM-CRF*                & 62.61 & \textbf{40.81} & 59.7\\ 
RoBERTa-KLM-REP-CRF*            & \textbf{62.72} & 40.15 & \textbf{62.56}\\ \hline
\end{tabular}
}
\caption{F1 scores for various datasets for Keyphrase Extraction}
\label{tab:ke_results}
\end{table}

\subsection{Keyphrase Extraction}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
We report performance of our models for Keyphrase Extraction task on Inspec \cite{inspec}, SemEval-2010 (SE10) \cite{kim-etal-2010-semeval}, and SemEval-2017 (SE17) \cite{augenstein2017semeval} datasets. \cite{sahrawat2019keyphrase} first explore keyphrase extraction as a sequence labelling task with contextual embeddings and demonstrate the effectiveness of a CRF for this task. Similarily we use the sequence classification paradigm to perform Keyphrase Extraction and we employ the sequence classification Token Classification Architecture implemented by \cite{wolf2020transformers} with an addition of a CRF in order to fine-train our different pre-trained models. We compare our results with RoBERTa+BiLSTM-CRF \cite{sahrawat2019keyphrase}, RoBERTa+TG-CRF \cite{tg-keyphrase-extraction} and RoBERTa+Hypertnet-CRF \cite{duan21_interspeech}, but different from these architectures we do not use an LSTM layer between the contextualized embeddings and the CRF. In line with \cite{sahrawat2019keyphrase} we fine-tune over 100 epochs with a batch size of 4 for all three datasets, with only a different learning rate of 5e-5. We see that our proposed architectures outperform state-of-the-art for Keyphrase Extraction by significant margins across all three datasets with fewer parameters than state-of-the-art models. While RoBERTa-extended, shows gains over RoBERTa+BiLSTM-CRF, this is expected since the domain of the continued pre-training data is more in line for Keyphrase Extraction evaluation. However, the models that learn more explicitly learn keyphrase representations significantly outperform RoBERTa-extended. We believe the anamolous results for SemEval-2010 are because of the size of the dataset, which is a fairly small dataset of 130 documents for training and 100 documents for testing. 

\begin{table*}[]
\scalebox{0.76}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\hline
    & \multicolumn{2}{c|}{Inspec} & \multicolumn{2}{c|}{NUS} & \multicolumn{2}{c|}{Krapivin} & \multicolumn{2}{c|}{SemEval} & \multicolumn{2}{c}{KP20k} \\ \hline
Model & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M \\ \hline
catSeq (Yuan et al., 2020) & 22.5 & 26.2 & 32.3 & 39.7 & 26.9 & 35.4 & 24.2 & 28.3 & 29.1 & 36.7\\ 
catSeqTG (Chen et al., 2019b) & 22.9 & 27 & 32.5 & 39.3 & 28.2 & 36.6 & 24.6 & 29.0 & 29.2 & 36.6\\ 
catSeqTG-2RF1 (Chan et al., 2019) & 25.3 & 30.1 & \textbf{37.5} & 43.3 & 30 & 36.9 & 28.7 & 32.9 & 32.1 & 38.6\\ 
GANMR (Swaminathan et al., 2020) & 25.8 & 29.9 & 34.8 & 41.7 & 28.8 & 36.9 & - & - & 30.3 & 37.8\\ 
ExHiRD-h (Chen et al., 2020) & 25.3 & 29.1 & - & - & 28.6 & 34.7 & 28.4 & 33.5 & 31.1 & 37.4\\ 
Transformer (Ye et al., 2021) & 28.15 & 32.56 & 37.07 & 41.91 & \textbf{31.58} & 36.55 & \textbf{28.71} & 32.52 & \textbf{33.21} & 37.71\\ \hline
%SETTRANS(ONE2SET) & 28.53 & 32.43 & \textbf{40.61} & \textbf{45.07} & \textbf{32.61} & \textbf{36.41} & 33.12 & 35.71 & \textbf{35.85} & \textbf{39.24} \\ \hline
BART* &  23.59 & 28.46 & \textbf{\textit{35.00}} & 42.65 & 26.91 & 35.37 & 26.72 & 31.91 & 29.25 & 37.51\\  
BART-KLM-REP-DOC* & 24.42 & 29.57 & 31.37 & 39.24 & 24.21 & 32.60 & 24.69 & 30.50 & 28.82 & 37.59\\ 
BART-KLM-REP-KG* & 24.49 & 29.69 & 34.77 & \textbf{43.57} & \textbf{\textit{29.24}} & \textbf{38.62} & \textbf{\textit{27.47}} & \textbf{33.54} & \textbf{\textit{30.71}} & \textbf{39.76} \\
BART-KLM-REP-KG* (no finetune) & \textbf{30.72} & \textbf{36.89} & 18.86 & 21.67 & 18.35 & 20.46 & 20.25 & 25.82 & 12.57 & 15.41 \\
\hline
\end{tabular}
}
\caption{Keyphrase Generation for Present Keyphrases. State-of-the-art is marked in \textbf{Bold} and our best performing models as \textbf{\textit{Bold-Italicized}}}
\label{tab:KG_Present_results}
\end{table*}

\begin{table*}[]
\scalebox{0.76}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\hline
    & \multicolumn{2}{c|}{Inspec} & \multicolumn{2}{c|}{NUS} & \multicolumn{2}{c|}{Krapivin} & \multicolumn{2}{c|}{SemEval} & \multicolumn{2}{c}{KP20k} \\ \hline
\textbf{Model} & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M & F1@5 & F1@M \\ \hline
catSeq (Yuan et al., 2020) & 0.4 & 0.8 & 1.6 & 2.8 & 1.8 & 3.6 & 1.6 & 2.8 & 1.5 & 3.2 \\ 
catSeqTG (Chen et al., 2019b) & 0.5 & 1.1 & 1.1 & 1.8 & 1.8 & 3.4 & 1.1 & 1.8 & 1.5 & 3.2 \\ 
catSeqTG-2RF1 (Chan et al., 2019) & 1.2 & 2.1 & 1.9 & 3.1 & 3.0 & 5.3 & \textbf{2.1} & \textbf{3.0} & 2.7 & \textbf{5.0} \\ 
GANMR (Swaminathan et al., 2020) & 1.3 & 1.9 & 2.6 & 3.8 & \textbf{4.2} & 5.7 & - & - & \textbf{3.2} & 4.5 \\ 
ExHiRD-h (Chen et al., 2020) & 1.1 & 2.2 & - & - & 2.2 & 4.3 & 1.7 & 2.5 & 1.6 & 3.2 \\ 
Transformer (Ye et al., 2021) & 1.02 & 1.94 & \textbf{2.82} & \textbf{4.82} & 3.21 & 6.04 & 2.05 & 2.33 & 2.31 & 4.61 \\ \hline
%SETTRANS(ONE2SET) & 2.11 & 3.43 & 4.22 & 6.04 & 4.77 & 7.31 & 2.63 & 34.5 & 3.62 & 5.83 \\ \hline
BART* & 1.08 & 1.96 & \textbf{\textit{1.80}} & \textbf{\textit{2.75}} & 2.59 & 4.91 & 1.34 & 1.75 & 1.77 & 3.56\\ 
KeyBART-DOC* & 0.99 & 2.03 & 1.39 & 2.74 & 2.40 & 4.58 & 1.07 & 1.39 & 1.69 & 3.38\\   
KeyBART* &  0.95 & 1.81 & 1.23 & 1.90 & \textbf{\textit{3.09}} & \textbf{6.08} & \textbf{\textit{1.96}} & \textbf{\textit{2.65}} & \textbf{\textit{2.03}} & \textbf{\textit{4.26}} \\
KeyBART* (no finetune) & \textbf{1.83} & \textbf{2.92} & 1.46 & 2.19 & 1.29 & 2.09 & 1.12 & 1.45 & 0.70 & 1.14 \\ \hline
\end{tabular}
}
\caption{Keyphrase Generation for Absent Keyphrases. State-of-the-art is marked in \textbf{Bold} and our best performing models as \textbf{\textit{Bold-Italicized}}.}
\label{tab:KG_Absent_results}
\end{table*}

\subsection{Keyphrase Generation}
We evaluate keyphrase generation performance on Inspec \cite{inspec}, NUS \cite{NUSDataset}, Krapivin \cite{krapivin2009large}, SemEval \cite{kim-etal-2010-semeval} and KP20K \cite{meng-etal-2017-deep}. The task is to generate the CatSeq output of the present and absent keyphrases for a given concatenated title and abstract, following previous work (Meng et al., 2017; Chen et al., 2019b,a; Yuan et al., 2020). We use the PresAbs ordering of the keyphrases as that was shown to the be the most effective representation in \cite{PresAbsCite}. Further, the models are fine-tuned only on the largest dataset, KP20k, for 300k steps with a batch size of 32 across 4 GPUs with a learning rate of 5e-5. Similar to \cite{KeyGenHyperParamCite} we use 50 beams for beam search and restrict our maximum generated sequence length to 40. For our evaluation we use macro-averaged F1@5 and F1@M in line with Chan et al., 2019 and Chen et al., 2020 for both present and absent keyphrase generation. F1@M evaluates all the keyphrases predicted by the model with the ground-truth keyphrases. F1@5, as the name suggests evaluates only the first 5 keyphrases, however when there are fewer than five keyphrases, random incorrect keyphrases are appended till it reaches five predictions. Chan et al. 2019, shows that without this appending F1@M is the same as F1@5, when predictions are fewer than five. In Table \ref{tab:KG_Present_results} and Table \ref{tab:KG_Absent_results} we see that BART-KLM-REP-KG is the most effective training method achieving state-of-the-art on most datasets for F1@M in present and absent keyphrase generation. We believe the perturbation of the input during the pre-training setup makes this model for robust and helps it identify and generate keyphrases more effectively. We also observe that our results for F1@5 aren't as competitive as F1@M and we believe this is because our model tends to favor predictig fewer than 5 keyphrases and thus tends to suffer from the random addition of keyphrases for F1@5. More concretely, in the SemEval dataset we have an average of 2.51 keyphrases predicted per document. Further, Yuan et al., 2021 also present a ONE2SET training paradigm and for a fair comparison we compare to their Transformer (ONE2SEQ) results, since we also train in the ONE2SEQ paradigm and not ONE2SET. 

\begin{table}[t]
\scalebox{0.9}{
\begin{tabular}{lccc}
\hline
\textbf{Model} & \textbf{R1} & \textbf{R2} & \textbf{RL} \\ \hline
%BART              & 44.16 & 21.28 & 40.9      \\ \hline
BART*             & 42.93 & 20.12 & 39.72 \\ 
KeyBART-DOC*  & 42.92 & 20.07 & 39.69  \\ 
KeyBART*   & \textbf{\textit{43.10}} & \textbf{\textit{20.26}} & \textbf{\textit{39.90}}  \\ \hline
\end{tabular}
}
\caption{Summarization results on CNN/DailyMail datasets. Our best performing models are marked as \textbf{\textit{Bold-Italicized}}}
\label{tab:summ_results}
\end{table}

\subsection{Summarization}
We run BART, BART-KLM-REP-DOC and BART-KLM-REP-KG on the CNN DailyMail \cite{cnn-dm}. Keyphrase Generation is also considered as an extreme form of summarization and hence hope to see gains in performance. We are unable to reproduce the original BART scores for R1, R2 and RLSum, so we use the reported hyperparameters to reproduce the results to best of our ability accounting for slight implementation differences in framework versions. We hope this provides a more fair comparison with our model results. We do not claim SOTA for summarization models, rather want to demonstrate that there are potential performance gains by training on a keyphrase specific objective. This is exemplified in Table \ref{tab:summ_results} where we see that the standard denoising autoencoder setup results in marginal losses, however training with the keyphrase generation objective actually improves the ROUGE scores across the board.


